Fine-Grained Human Feedback Gives Better Rewards for Language Model Training

Language models (LMs) often exhibit undesirable text generation behaviors, including generating false, toxic, or irrelevant outputs. Reinforcement learning from human feedback (RLHF) - where human preference judgments on LM outputs are transformed into a learning signal - has recently shown promise in addressing these issues. However, such holistic feedback conveys limited information on long text outputs; it does not indicate which aspects of the outputs influenced user preference; e.g., which parts contain what type(s) of errors. In this paper, we use fine-grained human feedback (e.g., which sentence is false, which sub-sentence is irrelevant) as an explicit training signal. We introduce Fine-Grained RLHF, a framework that enables training and learning from reward functions that are fine-grained in two respects: (1) density, providing a reward after every segment (e.g., a sentence) is generated; and (2) incorporating multiple reward models associated with different feedback types (e.g., factual incorrectness, irrelevance, and information incompleteness). We conduct experiments on detoxification and long-form question answering to illustrate how learning with such reward functions leads to improved performance, supported by both automatic and human evaluation. Additionally, we show that LM behaviors can be customized using different combinations of fine-grained reward models. We release all data, collected human feedback, and codes at https://FineGrainedRLHF.github.io.

==> content/abstract-old.tex <==
   % Feedback provision, a critical component in human learning, is also shown to be effective for training language models to achieve desirable generation outputs. Reinforcement learning with human feedback (RLHF) has recently shown promise in aligning language model generation with human-preferred attributes. However, challenges arise when evaluating the entirety of model outputs, particularly in long-form generation tasks. In this paper, we investigate the use of fine-grained human feedback as explicit training signals to train language models more effectively and efficiently compared to overall human preferences. We introduce a novel reinforcement learning algorithm that leverages multiple reward functions, addressing different types of undesired behavior and specificity levels in generated outputs. Our experiments on long-form question answering and unlearning toxicity tasks demonstrate the superiority of fine-grained reward-based training over preference-based reward in terms of effectiveness and data efficiency. Additionally, we show that using different reward models allows for better control over the training process and customization of desired behaviors. 

    %\raj{There's two dimensions of granularity here: (1) denser in the sequence level - toxicity ablations (singular bandit reward vs token MDP) is proof of this. (2) more fine grained in types of rewards in long form QA, splitup of diff types of rewards. (Intuitively this makes sense because the standard way of doing things in RLHF NLP is to just add all rewards up in one big number for the end of a sequence which loses info, what if one rew is negative and other is positive)}
    Language models (LMs) often exhibit undesirable behaviors, including generating false, toxic, or irrelevant outputs. 
    %\hanna{be more precise; your paper doesn't address toxic; only list properties that you can solve, like generating false, irrelevant, or redundant?} \nascomment{+1} 
    Reinforcement learning from human feedback (RLHF)---where human preference judgments on LM outputs are transformed into a learning signal---has recently shown promise in addressing these issues. However, such holistic feedback conveys limited information. For instance, it does not directly mark which aspect of the LM outputs yields the observed user preference; e.g., which part of an output contains what type(s) of errors. %\nascomment{seems to me there are two issues to be mentioned:  global/local (standard approach doesn't localize to particular tokens or subsequences) and different types of problems (e.g., toxicity vs. redundancy vs. other things)} 
    In this paper, we use fine-grained human feedback ( \hanna{instead of example, ulist the concrete fine-grained feedback that you have}\nascomment{+1}e.g., which sentence is false, which sub-sentence is irrelevant) as explicit training signal. 
    % We collect \DATASETNAME, a dataset of LM-generated text annotated with fine-grained human feedback, 
    We introduce \textit{\NAME}, an RL framework that enables LMs to learn from multiple reward models that are fine-grained in two dimensions: (1) providing reward densely after every small segment (e.g., a sentence) is generated; (2)  incorporating multiple rewards, each focusing on a specific feedback type (e.g., factual incorrectness, irrelevance, and information incompleteness). We conduct experiments on detoxification and long-form question answering to illustrate how learning with rewards at these two granularity dimensions leads to  improved performance, supported by both automatic and human evaluation. Additionally, we show that LM behaviors can be customized using different combinations of fine-grained reward models.
    We will release all data, collected human feedback and code. 


==> content/analysis.tex <==
\subsection{Analysis}
\label{sec:analysis}

\noindent{\bf Reward model performance}
- RM performance (dive into each individual RM model, and provides error analysis)

\noindent{\bf Error Analysis}
- generation error analysis for each error type, and how that related to the RM analysis findings above. Compare generation errors before and after RL training.


- Compare ChatGPT performance with ours; Hanna's suggestion: check whether our RMs can be generalized to bigger models like ChatGPT

==> content/data_rms.tex <==
\section{Data, Human Feedback, and Reward Models}
\label{sec:task_and_data}

\input{content/lfqa}

\input{content/detox}

==> content/exp.tex <==
\section{Main Results}

\nascomment{might be easier to follow the paper if you have two sections, one that gives all details about detox, and another on lfqa.  ``all the details'' means data, human feedback, reward models, experiments, analysis.  that way there's less flipping back and forth.  if you don't do that, you need to pick one ordering and always follow it (detox comes first here, but lfqa came first in section 3).  separating the two makes more sense if each leads to a different, complementary set of findings/conclusions}

In this section, we present experimental results for detoxification and long-form question answering tasks. We compare our proposed method, \textit{\NAME} with the initial policy model, RLHF with holistic rewards and other task-specific baselines. For the \textbf{detoxification} task (\S\ref{exp:ut}), we demonstrate that sentence-level fine-grained rewards exhibit greater sample efficiency compared to holistic rewards, achieving lower toxicity with fewer training steps while maintaining a similar level of fluency. For the \textbf{long-form question answering} task (\S\ref{exp:lfqa}), 
%we introduce three types of fine-grained reward models, each targeting a specific feedback type as described in \S\ref{sec:lfqa}. 
our \textit{\NAME} outperforms preference-based rewards in both automatic and human evaluations when using the three fine-grained reward models introduced in \S\ref{sec:lfqa}. Additionally, we conduct an in-depth analysis of the fine-grained reward models, revealing that they compete against each other and adjusting their weights during RL training leads to distinct behaviors in LM generation. We report model performance scores averaged over 3 runs with random seeds for each RL experiment.


% we present empirical results that show the effectiveness and data efficiency of training language models with fine-grained reward models, comparing to models trained with preference-based or full-sequence-based reward models or in a supervised training setting. We also compare with the generation outputs from ChatGPT [CITE] with the task instruction and in-context examples.

\subsection{Detoxification}
\label{exp:ut}

\paragraph{Experimental Setup} We use the decoder-only model GPT-2-base [CITE] as the initial policy $P_{\theta_{init}}$ since this is a continuous generation task. During both the exploration stage in RL training and inference, we use nucleus sampling decoding with $p$ = 0.9 and temperature = 1.0, following previous work on this task [CITE], and the generation length limit is set to 48. The value model used during RL training is also initialized with GPT-2-base. We report RL training parameters in Appendix.

\paragraph{Evaluation and Additional Compared Systems}
We report the toxicity score calculated on each full generation sequence from the \textsc{Perplexity} API, as well as other commonly used metrics for \textsc{RealToxicityPrompts}, including n-gram diversity and GPT-2 XL perplexity that indicates the generation fluency. The toxicity score is reported as the maximum score among 4 sampled model outputs, averaged over all test input prompts. Other metrics are reported as the average score of the same 4 samples. We also compare our model with \textsc{DExperts} [CITE], the best performing conditional generation model on \textsc{RealToxicityPrompts}.

\paragraph{Results}

- Main result table that shows better performance of using fine-grained reward, compared with using sequence-level reward

- Training step efficiency plot that shows using fine-grained reward is more efficient



\input{tables/toxicity}



\subsection{Long-Form Question Answering}
\label{exp:lfqa}

\paragraph{Experimental Setup} Our policy model is based on T5-large [CITE] and $P_{\theta_{init}}$ is supervisely fine-tuned on 1000 training examples, as explained in \S\ref{sec:lfqa}. During RL exploration, we use top-k ($k=20$) sampling decoding with temperature = 0.7, which is set based on previous RLHF work [CITE]. 
All reward models we use are based on Longformer-base [CITE]. The value model used during RL training is initialized with T5-base. We report RL training parameters in Appendix. During inference, we use greedy decoding to generate the responses. \el{explain why we do greedy instead of sampling as in detoxicification}

% \paragraph{Baselines}
% We compare three kinds of models. The first is supervised fine-tuning models. We include \textbf{SFT}, our policy initialization, and \textbf{SFT-4k}, in which we further fine-tune SFT on the full training set (4000 examples) with reference answers. The second is SFT tuned with preference-based reward, which we referred to as \textbf{RLHF}. Finally, SFT tuned with our fine-grained reward models is denoted as \textbf{Fine-Grained RLHF}.

\paragraph{Evaluation and Additional Compared Systems}
We use both automatic and human evaluations on the test set. For automatic evaluation, we report RougeLSum [CITE] as used for the original ASQA data, as well as the score from each fine-grained reward model (trained on all feedback we collect). 
%We discuss in Section??? that our fine-grained reward model correlates well with our human evaluation results.
For human evaluation, we use the same protocol of feedback collection to have the same set of workers to annotate each model output for (1) irrelevance, repetition and incoherence error and (2) ncorrect or unverifiable facts. Since we observe that it takes more time to annotate explicit missing information for every model, we ask human to compare each model pair for their information completeness. Human evaluation is conducted on 200 randomly sampled test examples, and each model output is sampled from inference results of 3 training runs. 


\paragraph{Results}
- Main result table that shows better performance of using fine-grained reward, compared with using sequence-level reward and supervised training, on both auto and human eval

- Annotation sample efficiency plot that shows using fine-grained reward is more efficient

- Main result table also shows that different combinations of RM weights lead to different RM optimizations (controllability) and we show qualitative examples in Section~\ref{sec:analysis}

- Ablations of removing each RM and how they compete with each other


\input{tables/human_evaluation}


\paragraph{Human Evaluation}


\input{tables/LFQA_automatic}

\paragraph{Automatic Evaluation}


\paragraph{Customization}

\paragraph{Reward Model Ablation}

\paragraph{Sample Efficiency}



% \begin{figure}[htbp]
%     \centering
%     \begin{minipage}{0.45\textwidth}
%         \centering
%         \caption{Main result table for LFQA}
%         \label{tab:table1}
%         \begin{tabular}{lccccc}
%             \toprule
%             \textbf{} & \textbf{Rouge} & \textbf{Rel} & \textbf{Fact} & \textbf{Comp} & \textbf{Len} \\
%             \midrule
%             SL & - & - & - & - & - \\
%             RLS & - & - & - & - & - \\
%             RLFG & - & - & - & - & - \\
%             \bottomrule
%         \end{tabular}
%     \end{minipage}\hfill
%     \begin{minipage}{0.45\textwidth}
%         \centering
%         \caption{Table 2}
%         \label{tab:table2}
%         \begin{tabular}{lcccc}
%             \toprule
%             \textbf{} & \textbf{Toxicity} & \textbf{PPL} & \textbf{Bi-Div} & \textbf{Tri-Div} \\
%             \midrule
%             RLS & - & - & - & - \\
%             RLFG & - & - & - & - \\
%             \bottomrule
%         \end{tabular}
%     \end{minipage}
% \end{figure}




==> content/exp_detox.tex <==
\section{Task 1: Detoxification}


The task of detoxicification aims to reduce the toxicity in the model generation $y$ when given a prompt $x$. We use
\textsc{RealToxicityPrompts}, which is a dataset of 100K sentence-level prompts derived from the web that are known to easily elicit problematic generations in models like GPT-2 [CITE]. Since toxicity is the only undesired behavior in this task, we only use one reward model to measure the generation toxicity. We follow previous work [CITE] to use GPT-2 as the initial model and \textsc{Perspective} API as the reward model, which is trained with millions of examples gathered from several online platforms and annotated by human annotators as toxic or not. That means we use an off-policy reward model that is not trained on outputs from the initial policy $P_{\theta_{init}}$.
When given a textual input, the API outputs a score between 0 (non-toxic) and 1 (toxic). To calculate the \textit{fine-grained reward}, we query the API after the model generates each sentence instead of generating the full sequence. For each generated sentence $y^s_j$, we assign \textsc{Perspective}($[y^s_1, \dots, y^s_j]$) - \textsc{Perspective}($[y^s_1, \dots, y^s_{j-1}]$) as the sentence reward. In the comparison experiment that uses the full-sequence reward during RL training, we simply query the API with the entire output $y$.
%\as{should we say something about how this is not really on-policy training because perspective was not trained on the generations from our initial model?}\nascomment{agree}
%\raj{Wait, on policy doesn't have anything to do rewards. PPO is on policy no matter what}
%\as{the reward functions are off-policy or at the very least OOD unlike in the other QA experiments where the reward functions are trained on the model's (previous) generations, making them on-policy. in the first case the reward function is policy-dependent because we are training it on model-generated outputs; in this case it is policy-independent and OOD}

\subsection{Experiments}
\label{sec:exp_detox}

We present experimental results for the detoxification task. We compare our proposed method, \textit{\NAME} with the initial policy model GPT-2, RLHF with holistic rewards and \textsc{DExperts} [CITE], the best performing conditional generation model on \textsc{RealToxicityPrompts}. We demonstrate that \textbf{sentence-level fine-grained rewards exhibit greater sample efficiency compared to holistic rewards}, achieving lower toxicity with fewer training steps while maintaining a similar level of fluency. We report model performance scores averaged over 3 runs with random seeds for each RL experiment.

\paragraph{Experimental Setup} We use the decoder-only model GPT-2-base [CITE] as the initial policy $P_{\theta_{init}}$ since this is a continuous generation \nascomment{what is a continuous generation task?} task. During both the exploration stage in RL training and inference, we use nucleus sampling decoding with $p$ = 0.9 and temperature = 1.0, following previous work on this task [CITE], and the generation length limit is set to 48. The value model used during RL training is also initialized with GPT-2-base. We report RL training parameters in Appendix.

\paragraph{Evaluation}
We report the toxicity score calculated on each full generation sequence from the \textsc{Perplexity} API, as well as other commonly used metrics for \textsc{RealToxicityPrompts}, including n-gram diversity and GPT-2 XL perplexity that indicates the generation fluency. The toxicity score is reported as the maximum score among 4 sampled model outputs, averaged over all test input prompts. Other metrics are reported as the average score of the same 4 samples. 


\input{tables/toxicity}

\paragraph{Results}
Table~\ref{fig:toxicity_result} shows the experimental results on \textsc{RealToxicityPrompts} test set. \nascomment{you need to explain the metrics a bit more} Besides PPO, we also compare our approach with state-of-the-art controlled generation approaches GeDi[CITE] and DEXPERT[CITE]. PPO with sentence-level fine-grained reward (PPO FG) attains both the lowest toxicity and perplexity among all methods.

\paragraph{RL with fine-grained reward is more sample efficient than holistic reward}
\nascomment{should be a figure, not a table} Table~\ref{fig:toxicity_curve} shows the max toxicity and perplexity on the development set during training. PPO with fine-grained reward makes toxicity drop much faster while keeping a low-level perplexity. This show that fine-grained reward is more sample efficient than holistic reward. One explanation is that fine-grained rewards locate where the toxic contents are, which is a stronger training signal compared with a scalar reward for the whole text. The cost is that we have to query the reward model more times per example.

==> content/exp_lfqa.tex <==
\section{Task 2: Long-Form Question Answering}
\label{sec:lfqa}
%We test out the effectiveness of training language models with fine-grained feedback on two tasks---long-form question answering and unlearning toxicity. In this section, we introduce the data, feedback and reward models we use for each task.

\nascomment{paragraph labels should be more parallel between the two task sections (e.g., there's no ``Task and Data'' for Task 1} \el{sorry Noah, I just started merging everything for each task to a single section, so the titles, etc can be a bit messy now..}


\paragraph{Task and Data} \hanna{LFQA is a bit too much; let's keep it as Long Form QA} LFQA requires generating a textual response to a question with comprehensive answers and explanations. ASQA is a dataset [CITE] that focuses on answering ambiguous factoid questions [CITE] in an open-domain setting. 
%ASQA provides the oracle knowledge contexts used for answering each question, and we use BM25 [CITE] to map each knowledge context to the closest passage from its provided Wikipedia passage corpus. 
We use their provided oracle knowledge contexts to reformulate the task into a reading comprehension setting: given the input $x$ that contains a question $q$ and a set of knowledge passages $P=\{p_1, \dots, p_{|P|}\}$, generate a long-form response $y$. On average, there are roughly 65 words in each gold response.
Since ASQA does not release the test set, we create our own train/development/test data splits from the original train and development sets.
% Our train and dev examples come from the original ASQA train set and our test examples are the original ASQA dev examples. 
We name our newly constructed data as XXX \as{is this the same as the dataset we are releasing with feedback? if not, then I'm not sure we need a new name for it} to differentiate it from the original ASQA. Overall, we have 3,853 training, 500 development and 948 test examples.\footnote{Data construction details are available in the Appendix.}

\paragraph{Initial Policy and Fine-Grained Human Feedback}
Before collecting human feedback, we follow [CITE] to initialize the policy model with supervised finetuning on a small set of examples. Specifically, we use T5-large [CITE] as the base LM \as{is ``base LM'' commonly understood to refer to an initial set of parameters when doing LLM fine-tuning?}\nascomment{could replace this with the symbol you proposed for initial model, I think it was $P_{\theta_{\text{init}}}$?} and use 1,000 training examples for supervised finetuning. We denote this initial policy model as \textbf{SFT}.
We then sample outputs from SFT for the remaining training and development examples \as{how do we use the dev examples here?}, and collect \textit{fine-grained} human feedback in three error categories--- {$C_1$}: irrelevance, repetition, and incoherence; {$C_2$}: incorrect or unverifiable facts based on knowledge passages; and {$C_3$}: incomplete information. \el{we need to either use names for ``error'' or ``desired behavior'' categories throughout the paper} 


%Then we collect feedback on a sampled output of T5-SFT for each one of the remaining 2,853 training examples and the 500 dev examples, using the Amazon Machanical Turk platform. 
We instruct workers to identify any errors in each model output \nascomment{again, deviates from ``$a$'' notation used earlier} $y = y_{1, \dots, T}$, marking the span of text associated with each identified error.
%mark textual spans within each model output $y=y_{1,\dots,T}$ of a length of T words, such that each span contains an error.
%, and mark the output as containing error $c_3$ if they find relevant information from the passages that is missing in $y$. 
Formally, we define the set of user-annotated feedback for a task prompt $x$ and model output $y$ as $\mathcal{F} = \{f_i\}$ where each $f_i=\langle c_{i}, b_i, e_i\rangle$ represents the user-identified span $y_{b_i,\dots,e_i}$ of the error category $C_{c_i}$, where $c_i\in \{1,2,3\}$.
%We design a qualification task to select qualified workers for this feedback annotation task. We constantly monitor the annotation process and send feedback to workers.
\as{we should have plain-language descriptions of these three restrictions} \nascomment{agree.  my reading here is that among the first two categories, spans can't overlap, if $C_2$ is present other annotations are forbidden, and $C_3$ can only apply to whole output sequences.  I think you can probably say this in precise English without math symbols.  later you say something about $C_2$ being sentence level but that's not here?} Importantly, we impose three restrictions in the annotation: (1) for any $i$ and $j$ where $i \neq j$, $c_i < 3$ and $c_j < 3$, the spans $y_{b_i,\dots,e_i}$ and $y_{b_j,\dots,e_j}$ have no overlap; (2) if a span $y_{b_i,\dots,e_i}$ is annotated to have error of type $C_1$, the worker does not need to provide feedback whether the span contains error of type $C_2$; (3) if $c_i = 3$, then $b_i=1$ and $e_i=T$, which means information incompletion of $y$ can only be assessed at the whole sequence level.
Additionally, we ask workers to rewrite $y$ into a corrected version $y'$ that addresses all annotated feedback $\mathcal{F}$.\footnote{The Appendix contains details about the feedback collection interface, instructions, and quality control.}

%Overall, among all error spans we collect, x\% of them are VI errors and the remaining y\% are FI errors. However, it is important to note that we instruct workers to label FI errors only for places that don't contain a VI error. z\% examples are labeled as incomplete (i.e., contain IN error). 
To analyze human-human agreement, a subset of 300 examples receive annotations from two distinct workers.
We observe that while exact agreement in error span boundaries is low, they achieve reasonably high agreement on whether each sub-sentence contains $C_1$ (?\% \as{is this agreement statistics? what does this mean exactly?}) and whether a sentence contains $C_2$ (?\%).\footnote{We use spaCy [CITE] to segment generated model outputs into sub-sentences. \nascomment{this is confusing; what is the (qualitative) criterion that spacy is supposedly using to break sentences into parts?}} 
%As a result, we adopt the sub-sentence- and sentence-level specificity for VI and FI error feedback. 
The agreement on whether a model output contains complete information or not ($C_3$) is ?\%. \nascomment{conventional approach to measuring agreement is Cohen's $\kappa$ score (for two annotators) or Fleiss' $\kappa$ score for more.  another is Krippendorff's $\alpha$.  these account for chance}


\paragraph{Fine-Grained Reward Models}
We train three separate reward models $R_{\phi_1}$, $R_{\phi_2}$, and $R_{\phi_3}$ for $C_1$, $C_2$, and $C_3$ error categories respectively. For the reason as discussed above, we train these three reward models at a specificity level of sub-sentence, sentence, and full sequence, respectively. We use Longformer [CITE] as the base model to handle long input sequences \nascomment{this is confusing; suggests you use one model for some data and another model for other data?  earlier you said you used T5.}.\footnote{We provide more design details of each reward model in the Appendix.}

\paragraph{Irrelevance, repetition, and incoherence.}{$R_{\phi_1}$} targets to predict whether each sub-sentence $y^s_j$ in $y=y^s_1 \dots y^s_L$ \as{we should define formally what we get from segmentation. I am assuming this is a concatenation of subsentences, right?} contains a $C_1$ type error \as{which error is this again?}, and thus we add a 2-class token-level classification layer on the top of the Longformer encoder.
The model input has the format of ``\texttt{question:} $q$ \texttt{answer:} \texttt{[sep]} $y^s_1$ \texttt{[sep]} $y^s_2$ \dots '', and we take the classification output at each \texttt{[sep]} token to indicate whether the following $y^s_j$ contains a $C_1$ error.
We do not add passages in the model input because, intuitively, the detection of $C_1$ errors does not depend on them.
To train $R_{\phi_1}$, we apply a token-level classification loss to each \texttt{[sep]} token before $y^s_j$, where its gold label $g_j$ is ``\texttt{has error}'' if there is a $f_i\in\mathcal{F}$ that has $y_{b_i,\dots,e_i}$ overlapped with $y^s_j$ and ``\texttt{no error}'' otherwise.

When $R_{\phi_1}$ provides reward during RL training as in Eq.~\ref{eq:reward}, we read a reward value $R_{\phi_1}(x, y^s_1,\dots, y^s_j)$ for every $y^s_j$ (i.e., $\mathcal{S}^1_y$ includes last tokens of each $y^s_j$ \as{what is $\mathcal{S}$?}).
We define $R_{\phi_1}(x, y^s_1,\dots, y^s_j)=+1$ if $R_{\phi_1}$ predicts that $y^s_j$ contains an error and $-1$ if not.
\as{abusing notation here a bit: R should be giving us a scalar reward, but we are also defining it as giving us token-level classifications}


\paragraph{Incorrect or unverifiable facts.} $R_{\phi_2}$ is developed for detecting $C_2$ error \as{which error is this?} at the sentence level in a similar way. 
The model input has the format of ``\texttt{question:} $q$ \texttt{context:} $p_1$ $p_2$ \dots \texttt{answer:} \texttt{[sep]} $y_1^s$ \texttt{[sep]} $y_2^s$ \dots '', where $p$'s denotes the grounding passages and $y^s_i$ represents the $i$th sentence in this case. \as{we are reusing notation to refer to both subsentences and sentences, which may be confusing}
We train $R_{\phi_2}$ similarly as $R_{\phi_1}$, with one exception: as we instruct the workers not to annotate $C_2$ error for a span that is already labeled as containing $C_1$ error, we do not train \bm{$R_{\phi_2}$} on sentences that are labeled as containing $C_1$ but not $C_2$.


\paragraph{Incomplete information.} $R_{\phi_3}$ is trained to measure the informativeness ($C_3$) of $y$, at the full sequence level.
Instead of casting this as a classification task, $R_{\phi_3}$ maps each example to a single scalar reward. \as{I find this description rather confusing. can we start with an intuition and overview of what we are doing, perhaps with reference to related work, then formalize it?} \raj{suggestion: cite https://arxiv.org/abs/1909.03087 as a reason why we know preference feedback is more reliable than classification or likert scales but classification is easier to collect for this use case so we bootstrap pref style feedback from the classification esque data} We first construct the set of passage sentences $\mathcal{S}$ that are considered as containing all relevant information to the question $q$ by matching each sub-sentence in the corrected model output $y'$ to the closest passage sentence.\footnote{We observe frequent extractive behaviors from the initial policy model.} We then sample four responses from SFT, for each we do the same sentence matching to get a set of matched passages sentences $\mathcal{S}'$. We calculate $|\mathcal{S}' \cap \mathcal{S}|/|\mathcal{S}|$ as the informativeness score for each model response. Instead of training the model to predict the exact computed score, we follow [CITE] to pair up sampled responses for $q$ and denote each sampled response pair as ($y_p$, $y_l$), where $y_p$ has a higher score than $y_l$. We drop the pairs where the two responses have the same score. Then we train $R_{\phi_3}$ with the following loss function: 
\begin{equation}
\label{eq:pref-rm-loss}
    \mathcal{L}_r(\phi)=-\mathbb{E}_{(x,y_p,y_l)\sim D} \Big[\log\big(\sigma(R_{\phi_3} (x, y_p) - R_{\phi_3} (x, y_l))\big)\Big]
\end{equation}
where $D$ is the set of model response pairs. During inference, $R_{\phi_3} (x, y)$ is used as the reward for the full response.


\paragraph{Preference-Based Human Feedback and Reward Model} 
For comparison purposes, we follow [CITE] to collect pairwise \textit{human preferences} from the same group of workers. We sample four model outputs for each prompt $x$, which gives 6 pairs of model outputs. We ask the workers to indicate pairwise preferences (ties are allowed) based on any errors of $C_1$, $C_2$, and $C_3$ they found in each model output. \as{do we have them annotate all 4 outputs for the error categories?} \el{No, that's just a preference for the overall quality}

The preference-based reward model has the same model architecture as $R_{\phi_3}$. It outputs a scalar score for a model response that represents the overall response quality. It is trained with the same loss function formulation as Eq~\ref{eq:pref-rm-loss}, with $y_p$ representing the human preferred response against $y_l$.

\paragraph{Annotation Details}
On average, both annotation tasks of fine-grained and preference feedback for one question take a worker about 6 minutes to finish. In contrast, [CITE] report that they spend about 15 minutes to label a human-written response for each question \as{what are we trying to say here? that it's faster to get feedback on model-generated outputs than to get human-written gold data? or something else}. \el{Yeah that's the idea, do you think this is a reasonable claim?} \raj{yes, just say it explicitly} On average, we pay \$1.65 per example for both tasks, which gives an \$16.5 hourly pay for our workers. We include details of the pay structure in Appendix.




\subsection{Experiments}
\label{sec:exp_lfqa}

We present experimental results for the long-form question answering task. We compare our proposed method, \textbf{\textit{\NAME}} \nascomment{use boldface consistently throughout the paper} with the initial T5 policy model trained with 1K examples (\textbf{SFT}) and RLHF with holistic rewards (\textbf{Preference RLHF}). The reward models used in RLHF experiments are trained on 2.8K examples with annotated feedback (but no gold human answer). For analysis, we also collect the human gold answers for these examples and use them to fine-tune a fully supervised T5 model (\textbf{SFT-Full}). Notice that SFT-Full requires much higher annotation costs because it takes longer (15 minutes per example) for annotators to draft long-form answers.

\nascomment{this paragraph seems to be a sketch of the section, not a reporting of the results.  the last few sentences promise some things but I don't know where to find them ... if this is meant to be a roadmap paragraph, put it at the front of the section and include section references} \textbf{\textit{\NAME}} outperforms \textbf{Preference RLHF} and \textbf{SFT} in both automatic and human \nascomment{aren't those in the next section? one thing at a time} evaluations when using the three fine-grained reward models introduced in \S\ref{sec:lfqa}. Surprisingly, it also outperforms \textbf{SFT-Full}, the fully-supervised model that requires considerably more annotation costs.
We conduct an in-depth analysis of the fine-grained reward models, revealing that they compete against each other, and adjusting their weights during RL training leads to distinct behaviors in LM generation. We also provide a qualitative analysis of reward model performance and its impact on the resulting policy model. 

\paragraph{Experimental Setup} Our policy model is based on T5-large [CITE] and $P_{\theta_{init}}$ is supervisedly finetuned on 1000 training examples, as explained in \S\ref{sec:lfqa}. During RL exploration, we use top-k ($k=20$) sampling decoding with temperature = 0.7, which is set based on previous RLHF work [CITE]. 
All reward models we use are based on Longformer-base [CITE]. The value model used during RL training is initialized with T5-base. We report RL training parameters in Appendix. The reward model weights we used in \NAME are $w_1=0.3, w_2=0.5, w_3=0.3$, unless otherwise specified. During inference, we use greedy decoding to generate the responses. \el{explain why we do greedy instead of sampling as in detoxicification} All scores  reported are averaged over 3 independent runs.

% \paragraph{Baselines}
% We compare three kinds of models. The first is supervised fine-tuning models. We include \textbf{SFT}, our policy initialization, and \textbf{SFT-4k}, in which we further fine-tune SFT on the full training set (4000 examples) with reference answers. The second is SFT tuned with preference-based reward, which we referred to as \textbf{RLHF}. Finally, SFT tuned with our fine-grained reward models is denoted as \textbf{Fine-Grained RLHF}.

\subsection{Human Evaluation Results}
\label{sec:exp:human_eval}

We conduct a human evaluation on the test set of \DATASETNAME to compare \textit{Fine-Grained RLHF} with all baselines. We use the same protocol of feedback collection to have the same set of workers  annotate each model output for \errIrr[(1) irrelevance, repetition, and incoherence error] and \errFact[(2) incorrect or unverifiable facts]. \nascomment{need to explain what you're measuring} Table~\ref{tab:human_1} shows the evaluation results \nascomment{text in graphs is too small.  this is a figure, not a table.  need to use consistent names everywhere (graph says conciseness, caption says relevance, the table says ``informativeness'' while main text says ``incompleteness''}. Here we report the error rate, which is measured by the percentage of sub-sentences that include an error span with a corresponding error. Notice that in our annotation protocol, there are no overlapping error spans, thus \errFact[factual errors] that inside \errIrr[relevance errors] are not counted. Table~\ref{tab:human_missing_answer} shows the results for \errMiss[information incompleteness]. Since we observe that it takes more time to annotate explicit missing information for every model, we ask annotators to compare each model pair for their information completeness. Human evaluation is conducted on 200 randomly sampled test examples, and each model output is sampled from inference results of 3 training runs.  \nascomment{put these details before the results, not after}



\input{tables/human_evaluation} 


\paragraph{\NAME outperforms Preference RLHF on all error types.} 
Table~\ref{tab:human_1} and~\ref{tab:human_missing_answer} show that our \NAME contains fewer sub-sentences that are \errIrr[irrelevant] to the question, much fewer \errFact[factual errors], and is more \errMiss[informative] compared with SFT and Preference RLHF. In the meantime, Preference RLHF, despite greatly reduces factual errors via RLHF, sacrifices conciseness and produces more sentences that are irrelevant to the question. \NAME outperforms Preference RLHF because it provides stronger and more detailed training signals.

\paragraph{\NAME outperforms SFT-Full on factuality and informativeness, despite much lower annotation cost.}
Surprisingly, we find that our \NAME also outperforms SFT-Full on \errFact[factuality] and \errMiss[informativeness], while being a little \nascomment{quantify} more verbose \nascomment{than one of the models?}. Notice that SFT-Full introduces a much higher annotation cost than our approach. (On average, drafting a gold answer takes 15 minutes per example, while fine-grained feedback takes 6 minutes) Also, RLHF is applicable to large amounts of unlabeled user inputs while supervised finetuning cannot.

\paragraph{RLHF is particularly effective in reducing factual errors.} From Table~\ref{tab:human_1}, we can see that both \NAME and Preference RLHF are effective in reducing \errFact[factual] errors in model generation. This agrees with findings in prior works [CITE] \nascomment{what did those papers find exactly?}. Meanwhile, we see little improvement in reducing \errIrr[type-1 errors]. Notice that \NAME is able to reduce such errors \nascomment{this seems to contradict the last sentence}, however, we observe that it will sacrifice LM's informativeness. \nascomment{complete sentence here} More discussion in \S~\ref{sec:exp:customization} and~\ref{sec:exp:reward}.


\subsection{LM Customization with \NAME}
\label{sec:exp:customization}

Since \NAME supports multiple reward models, adjusting their weights during RL leads to different LM behaviors. This fits users with diverse needs. For example, some users may want succinct answers, while others prefer longer and more complete answers. Due to the high cost of human evaluation, we first \nascomment{this would be easier to follow if you start of saying what you expect to see (a hypothesis), in plain English, before getting into the details.  I think this section can be more brief} introduce our automatic evaluation and then explores \NAME's ability on LM behavior customization.

\input{tables/LFQA_automatic}



\paragraph{Automatic evaluation}
We report RougeLSum [CITE] as used for the original ASQA data, as well as the score from each fine-grained reward model (trained on all feedback we collect). Table~\ref{tab:automatic_eval} shows automatic evaluation results on \NAME and all baselines on \DATASETNAME test set. As discussed in \S~\ref{sec:lfqa}, $R_{\phi_1}$, $R_{\phi_2}$, and $R_{\phi_3}$ reflect LM's \errIrr[conciseness], \errFact[factuality], and \errMiss[informativeness]. We can draw similar conclusions from Table~\ref{tab:automatic_eval} and human evaluation. \NAME outperforms all other methods on all error types.

\paragraph{LM Customization}
As in Table~\ref{tab:customization}, we explore three configurations of reward models and name them `short', `medium', and `long' according to the LM's average generation length. Let the weights for $R_{\phi_1}$, $R_{\phi_2}$, and $R_{\phi_3}$ be $w_1$, $w_2$, and $w_3$. For all configurations, we use $w_2=0.5$ and $w_3=0.3$. For `short', we use $w_1=0.4$, for `medium', we use $w_1=0.3$, and for `long', we use $w_1=0.2$. We can see that `short' get the shortest answer length, highest \errIrr[conciseness], but is also the lowest on other rewards. This configuration is suitable for users that want succinct answers. `Long', on the contrary, has the longest generation outputs and the most \errFact[factuality] and \errMiss[informativeness] reward. This reflects that LM is referencing a large amount of content from passages. The `medium' configuration balances three rewards and has the highest Rouge score compared with human-written answers. Qualitative results of LM customization are in Appendix.

\paragraph{Trade-off between error types}
We observe that the greater $w_1$, the bigger \errIrr[conciseness] reward, the smaller \errFact[factuality] and \errMiss[informativeness] rewards, and the shorter the generated outputs. One interpretation is that $R_{\phi_1}$ penalizes text spans that are irrelevant to the questions. As such, it encourages answering the question directly and penalizes referencing passages and auxiliary information. This reduces model generation lengths and informativeness and induces more factual errors.


\subsection{Reward Model Analysis}
\label{sec:exp:reward}

We further explore the relationship between reward models and how they impact policy model behavior. We conduct ablation studies \nascomment{too vague, what are you ablating exactly?  what do you expect to see?} on the validation set and report the automatic evaluation scores in Table~\ref{tab:reward_ablation}. Notice that the validation set only contains one reference answer per example, thus the Rouge score is lower than the test set.

\input{tables/reward_ablation}


\paragraph{Reward models are competing against each other.}
In the prior section, we find that there is a trade-off between each error type. To further look into this phenomenon, we explore the dynamics of each reward during training. Table~\ref{fig:reward_curve} shows each reward model's rewards on the validation set during training. All rewards are z-normalized for visualization. We see that \errFact[factuality] is consistently increasing. \errIrr[Conciseness] increases rapidly in the first 250 steps and then starts decreasing. \errMiss[Informativeness] exhibits an opposite trend, decreasing at first and then start increasing. As discussed earlier, one interpretation is that conciseness and informativeness are adversarial objectives, so the rewards are competing. Three rewards reach an equilibrium point in later steps. \nascomment{this is interesting but it's a little hard to understand; does higher conciseness reward mean the model is generating more concise answers?  or that the gold-standard answers are getting higher rewards for being concise?}


\paragraph{Ablation: why do we need three reward models?}
Table~\ref{tab:reward_ablation} explores the policy LM behavior when one of the three reward models is removed during training. Qualitative examples are in Appendix. First, we observe that the corresponding reward decreases dramatically when the model is removed. 
When the \errIrr[conciseness] reward model ($R_{\phi_1}$) is removed, the outputs become extremely long and the informative reward is extremely high. We observe the outputs and find the model is copying a lot of content from the passages.
When the \errFact[factual] reward model ($R_{\phi_2}$) is removed, the conciseness reward becomes the highest. We observe that the LM tends to answer the question directly and not reference the passages, which causes a lot of hallucinations.
When the \errMiss[informativeness] reward model ($R_{\phi_3}$) is removed, the output is the shortest among all configurations. The model is concise and factual but not providing all relevant information to the question. \nascomment{do we take this to mean that the reward functions are learning what we want them to learn?  that's a good question but you need to ask it explicitly before you start showing experiments}


\paragraph{Reward Model Performance \& Error Analysis}

\nascomment{this is all very hard to follow. explain the question you're trying to answer before saying what the results are}
The reward model $R_{\phi_1}$ for irrelevance, repetition, and incoherence error, has the binary classification accuracy of 69.6 and the F1 score (for the ``\texttt{has error}'' class) of 68.5. We sample 20 sub-sentences from the dev set where the $R_{\phi_1}$ predicts the opposite label to what the worker annotates, and observe that all of them either 1) contain relevant auxiliary information and is marked as ``\texttt{no error}'' by the worker or 2) are marked as irrelevant by the worker but provide closely related background information. In other words, $R_{\phi_1}$ is mostly struggling with predicting the relevance of auxiliary information, and it rarely fails to predict a direct answer as ``\texttt{has error}''. \el{provide evidence that the policy is learning from it; e.g., is able to generate more direct answers; as well as evidence that the policy is generating less aux info, etc}

The reward model $R_{\phi_2}$ for detecting incorrect or unverifiable facts has the accuracy of 77.8 and the F1 score of 67.5. We sample 20 sentences from the dev set where $R_{\phi_2}$ makes a prediction mistake and we observe that the mistakes often happen when the generated sentence is highly abstractive instead of directly copying information from the passage, or pieces multiple passage sentences together. We also observe that more than 80\% human labeled factual consistency errors occur when the model generates a direct answer to the question while the answer is hallucinated or a random entity from a passage. We notice that $R_{\phi_2}$ is able to correctly capture more than 80\% of such errors. \el{provide evidence that the policy is learning from it; e.g., is able to avoid the dominating errors; exhibit more extractive behaviors, etc; as well as evidence that the policy is generating less abstractive content for those that requires multi-hop reasoning}

The reward model for missing info $R_{\phi_3}$ gives an accuracy of 70.9 in pairwise comparison. We sample 20 pairs of model outputs and observe ?\% of them exhibiting clear quality difference. However, the effect of adding $R_{\phi_3}$ is not obvious based on results in Table ? (ablation of removing $R_{\phi_3}$) potentially due to the reasons discussed above.  

The preference-based reward model reaches an accuracy of 57.2 in pairwise comparisons, which is close to human-human agreement (60\% \el{confirm}). However, among 20 sample pairs of model outputs, we only observe ?\% of them exhibiting clear quality difference, which confirms our intuition that assessing long-form generation outputs holistically is a rather ambiguous and subjective task. This is also evidenced by the worse performance of Preference RLHF compared to Fine-Grained RLHF.


- Compare ChatGPT performance with ours; Hanna's suggestion: check whether our RMs can be generalized to bigger models like ChatGPT


% \begin{figure}[htbp]
%     \centering
%     \begin{minipage}{0.45\textwidth}
%         \centering
%         \caption{Main result table for LFQA}
%         \label{tab:table1}
%         \begin{tabular}{lccccc}
%             \toprule
%             \textbf{} & \textbf{Rouge} & \textbf{Rel} & \textbf{Fact} & \textbf{Comp} & \textbf{Len} \\
%             \midrule
%             SL & - & - & - & - & - \\
%             RLS & - & - & - & - & - \\
%             RLFG & - & - & - & - & - \\
%             \bottomrule
%         \end{tabular}
%     \end{minipage}\hfill
%     \begin{minipage}{0.45\textwidth}
%         \centering
%         \caption{Table 2}
%         \label{tab:table2}
%         \begin{tabular}{lcccc}
%             \toprule
%             \textbf{} & \textbf{Toxicity} & \textbf{PPL} & \textbf{Bi-Div} & \textbf{Tri-Div} \\
%             \midrule
%             RLS & - & - & - & - \\
%             RLFG & - & - & - & - \\
%             \bottomrule
%         \end{tabular}
%     \end{minipage}
% \end{figure}


==> tables/customization.tex <==
\begin{figure*}[h]
\footnotesize
    \centering
    \begin{minipage}{1.0\textwidth}
        \centering
        \small
        \scalebox{.8}{
        \begin{tabular}{lccc|ccccc}
            \toprule[1.2pt]
            & \multicolumn{3}{c}{Reward Weights} & \multicolumn{5}{c}{Automatic Evaluations} \\
            & $w_1$ & $w_2$ & $w_3$ & $R_{\phi_1}$   & $R_{\phi_2}$   & $R_{\phi_3}$  & Rouge & Len \\
            \midrule
            \multicolumn{9}{l}{\textbf{Customization}} \\
            $\ \ $Balanced & 0.3 & 0.5 & 0.3 \\
            $\ \ $Short  & 0.4 & 0.5 & 0.3\\
            $\ \ $Long  & 0.2 & 0.5 & 0.3\\
            \bottomrule[1.2pt]
        \end{tabular}
        }
        \caption{Customization and ablation}
    \end{minipage}
    
\end{figure*}
